In&Out : Diverse Image Outpainting via GAN Inversion

Image outpainting seeks for a semantically consistent extension of the input image beyond its available content. Compared to inpainting -- filling in missing pixels in a way coherent with the neighboring pixels -- outpainting can be achieved in more diverse ways since the problem is less constrained by the surrounding pixels. Existing image outpainting methods pose the problem as a conditional image-to-image translation task, often generating repetitive structures and textures by replicating the content available in the input image. In this work, we formulate the problem from the perspective of inverting generative adversarial networks. Our generator renders micro-patches conditioned on their joint latent code as well as their individual positions in the image. To outpaint an image, we seek for multiple latent codes not only recovering available patches but also synthesizing diverse outpainting by patch-based generation. This leads to richer structure and content in the outpainted regions. Furthermore, our formulation allows for outpainting conditioned on the categorical input, thereby enabling flexible user controls. Extensive experimental results demonstrate the proposed method performs favorably against existing in- and outpainting methods, featuring higher visual quality and diversity.

==> tex/4-fig_ablation.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{img/arch/arch_v4.pdf}
    \includegraphics[width=.95\linewidth]{img/placeholder.png}
    \caption{
    %
    \textbf{Ablation.}
    %
    }
    \vspace \figmargin
    \label{fig:ablation}
\end{figure}

==> tex/4-fig_irregular.tex <==
\begin{figure}[h!]
\vspace{-3mm}
\begin{minipage}[l]{0.49\linewidth}
%\begin{figure}[h!]
    \centering
    \includegraphics[width=.93\linewidth]{img_reb/reb-irr_mask_v1.pdf}
    \vspace{-3mm}
    \caption{
    %
    \textbf{Irregular case.}
    %
    }
    \vspace{-1mm}
    \label{fig:reb_irregular}
%\end{figure} 
\end{minipage}
\begin{minipage}[l]{0.49\linewidth}
%\begin{figure}[h!]
    \centering
    % \includegraphics[width=.8\linewidth]{img_sup/supp-fail_v0.pdf}
    % \includegraphics[width=\linewidth, height=2cm]{img_reb/reb-church_v1.pdf}
    \includegraphics[width=.93\linewidth]{img_reb/reb-church_v1.pdf}
    \vspace{-3mm}
    \caption{
    %
    \textbf{Structured case.}
    %
    }
    \vspace{-1mm}
    \label{fig:reb_structure}
%\end{figure} 
\end{minipage}
\end{figure}

\vspace{-3mm}

==> tex_sup/6-supp_gau_ablation.tex <==
\begin{figure*}[h!]
    \centering
    % \includegraphics[width=\linewidth]{img_sup/no_prior.pdf}
    % \includegraphics[width=\linewidth]{img_sup/supp-no_prior_v0.pdf}
    \includegraphics[width=.6\linewidth]{img_sup/supp-no_prior_v1.pdf}
    \caption{
    %
    \textbf{Qualitative ablation on using $\mathcal{L}_{\mathrm{prior}}$.} We show that, if without $\mathcal{L}_{\mathrm{prior}}$, the inversion has the risk in overfitting to the reconstruction loss with latents codes extremely far away from the training distribution. 
    %
    The outpainted area (right part of the image) may result in direct replication of the input image.
    %, as the latent code itself carries all the structural information without utilizing the generator feature in a valid way (\ie with values in the training distribution).
    %
    In contrast, by adding the $\mathcal{L}_{\mathrm{prior}}$,
    % the additional loss regularizes the final latent codes to be located in the training distribution (\ie within a Gaussian distribution). We show that this results in a significantly better visual quality and semantically reasonable outpainting results without replicating the input image.
    we show that the outpainting results produce significantly better visual quality and semantically reasonable outpainting results without replicating the input image.
    }
    \vspace \figmargin
    \label{fig:gaussian_qual}
\end{figure*} 

==> tex_sup/6-supp_more_single.tex <==
\begin{figure*}[t!]
    \centering
    % \includegraphics[width=\linewidth]{img/arch/arch_v4.pdf}
    \includegraphics[width=\linewidth]{example-image-a}
    \caption{
    %
    \textbf{More inversion results.} 
    }
    \vspace \figmargin
    \label{fig:more_single}
\end{figure*} 
